Auxiliary Variables for Multi-Dirichlet Priors

Bayesian models that mix multiple Dirichlet prior parameters, called Multi-Dirichlet priors (MD) in this paper, are gaining popularity. Inferring mixing weights and parameters of mixed prior distributions seems tricky, as sums over Dirichlet parameters complicate the joint distribution of model parameters. This paper shows a novel auxiliary variable scheme which helps to simplify the inference for models involving hierarchical MDs and MDPs. Using this scheme, it is easy to derive fully collapsed inference schemes which allow for an efficient inference.

==> bib.tex <==
@incollection{teh2010,
  author = {Teh, Yee Whye},
  booktitle = {Encyclopedia of Machine Learning},
  editor = {Sammut, Claude and Webb, Geoffrey I.},
  ee = {http://dx.doi.org/10.1007/978-0-387-30164-8_219},
  interhash = {30b0cea36d49d35f68fe52de068f6b75},
  intrahash = {068dee95886fe18deff5a95330b466ec},
  isbn = {978-0-387-30768-8},
  pages = {280-287},
  publisher = {Springer},
  title = {Dirichlet Process.},
  url = {http://dblp.uni-trier.de/db/reference/ml/ml2010.html#Teh10},
  year = 2010
}
@inproceedings{yano2010s,
  title={What's Worthy of Comment? Content and Comment Volume in Political Blogs.},
  author={Yano, Tae and Smith, Noah A},
  booktitle={ICWSM},
  year={2010}
}

@inproceedings{goel2016social,
  title={The Social Dynamics of Language Change in Online Networks},
  author={Goel, Rahul and Soni, Sandeep and Goyal, Naman and Paparrizos, John and Wallach, Hanna and Diaz, Fernando and Eisenstein, Jacob},
  booktitle={International Conference on Social Informatics},
  pages={41--57},
  year={2016},
  organization={Springer}
}

@inproceedings{kling2014detecting,
  title={Detecting non-gaussian geographical topics in tagged photo collections},
  author={Kling, Christoph Carl and Kunegis, J{\'e}r{\^o}me and Sizov, Sergej and Staab, Steffen},
  booktitle={Proceedings of the 7th ACM international conference on Web search and data mining},
  pages={603--612},
  year={2014},
  organization={ACM}
}

@inproceedings{schein2016poisson,
  title={Poisson-Gamma dynamical systems},
  author={Schein, Aaron and Wallach, Hanna and Zhou, Mingyuan},
  booktitle={Advances in Neural Information Processing Systems},
  pages={5006--5014},
  year={2016}
}

@article{teh06,
  added-at = {2011-05-09T23:10:52.000+0200},
  author = {Teh, Y. W. and Jordan, M. I. and Beal, M. J. and Blei, D. M.},
  biburl = {http://www.bibsonomy.org/bibtex/2d27d1177993c8e89c2fe5617c9ac4d49/josephausterwei},
  interhash = {34e30f6d1538ed136344f6a9cf8a791b},
  intrahash = {d27d1177993c8e89c2fe5617c9ac4d49},
  journal = {J. of the American Statistical Association},
  keywords = {imported},
  pages = {1566-1581},
  timestamp = {2011-05-09T23:10:52.000+0200},
  title = {Hierarchical {D}irichlet processes},
  volume = 101,
  year = 2006
}

@inproceedings{teh08b,
  added-at = {2010-10-11T23:06:25.000+0200},
  author = {Teh, Yee Whye and Kurihara, Kenichi and Welling, Max},
  biburl = {http://www.bibsonomy.org/bibtex/29caea939666373dcf8472bf0c5ed76eb/kurtmiller},
  booktitle = {Advances in Neural Information Processing Systems (NIPS)},
  interhash = {66b17a5b20bed0f5aa8c9dc71483919d},
  intrahash = {9caea939666373dcf8472bf0c5ed76eb},
  keywords = {imported},
  timestamp = {2010-10-11T23:06:32.000+0200},
  title = {Collapsed Variational Inference for {HDP}},
  year = 2008
}

@inproceedings{teh_07,
  added-at = {2009-10-23T10:55:58.000+0200},
  author = {Teh, Y. W. and Newman, D. and Welling, M.},
  biburl = {http://www.bibsonomy.org/bibtex/269de96cd53db5847a70206778565cff9/folke},
  booktitle = {Advances in Neural Information Processing Systems},
  interhash = {76dd3259e314bd00f4759b7891805df1},
  intrahash = {69de96cd53db5847a70206778565cff9},
  keywords = {collapsed inference lda variational},
  owner = {gregor},
  timestamp = {2009-10-23T10:58:25.000+0200},
  title = {A Collapsed Variational {B}ayesian Inference Algorithm for Latent
	{D}irichlet Allocation},
  volume = 19,
  year = 2007
}

